A Distributed Mincut/Maxflow Algorithm Combining Path Augmentation and Push-Relabel

We develop a novel distributed algorithm for the minimum cut problem. We primarily aim at solving large sparse problems. Assuming vertices of the graph are partitioned into several regions, the algorithm performs path augmentations inside the regions and updates of the push-relabel style between the regions. The interaction between regions is considered expensive (regions are loaded into the memory one-by-one or located on separate machines in a network). The algorithm works in sweeps - passes over all regions. Let $B$ be the set of vertices incident to inter-region edges of the graph. We present a sequential and parallel versions of the algorithm which terminate in at most $2|B|^2+1$ sweeps. The competing algorithm by Delong and Boykov uses push-relabel updates inside regions. In the case of a fixed partition we prove that this algorithm has a tight $O(n^2)$ bound on the number of sweeps, where $n$ is the number of vertices. We tested sequential versions of the algorithms on instances of maxflow problems in computer vision. Experimentally, the number of sweeps required by the new algorithm is much lower than for the Delong and Boykov's variant. Large problems (up to $10^8$ vertices and $6\cdot 10^8$ edges) are solved using under 1GB of memory in about 10 sweeps.

==> tex/old.tex <==
\section{Old}
%
%


%Input: Preflow $f$ on $E_R$, labeling $d$ on $B(R)$.
%\newline
%Output:Preflow $f$ on $E_R$ and labeling $d$ on $R\cup B(R)$ stable on $R$.
%\par
%Augmenting paths may be applied to a preflow network directly. We will augment from nodes with excess to the sink and also to boundary nodes. To achieve a stable preflow-labeling we will augment always from nodes with higher label to nodes with a lower label. 
%\par

%\begin{lemma}
%Let $P$ be augmenting $s\rightarrow t$ path in $G$ and let $G'$ be a residual network after augmenting on $P$. If there is no $s\rightarrow w$ path in $G$ then there is no $s\rightarrow w$ path in $G'$.
%\end{lemma}
%\begin{proof}
%Let $S=\{$vertices reachable from $s$ in $G$ $\}$. Since $w$ is not reachable, set $S$ describes $s$-$w$ cut of cost $0$ in $G$. The path $P$ can not contain vertices in $\bar S$ (as they are not reachable from $s$). Therefore augmenting on $P$ cannot push flow on edges $(\bar S, S)$ and hence cannot increase residual capacities $(S, \bar S)$, therefore $S$ remains $0$ $s$-$w$ cut in $G'$ and the statement of Lemma follows. Similarly, if there is no $w\rightarrow t$ path in $G$ than after augmentation on any path $s\rightarrow t$, no $w\rightarrow t$ path can appear.
%\end{proof}
%
%\begin{lemma}
%Let $W$ be set of nodes, from which $w\in V$ is reachable by a path in $G$, $W = \{v\mid \exists v\rightarrow w\}$. Let $s\notin W$. Then augmenting on paths $s\rightarrow t$ does not change $W$.
%\end{lemma}
%\begin{proof}
%A path $P$ from $s$ to $t$ does not contain vertices from $W$ (otherwise $w$ would be reachable form $s$). Therefore augmenting on $P$ cannot change the flow and, consequently, residual capacities on edges $(V, W)$.
%\end{proof}
%%
%Clearly, the following dual statement also holds true.
%\begin{lemma}
%Let $W$ be set of nodes reachable from $w\in V$ and $t\notin W$, $W=\{v\mid \exists w\rightarrow v\}$. Then augmenting on paths $s\rightarrow t$ does not change $W$.
%\end{lemma}
%\begin{proof}
%A path $P$ from $s$ to $t$ does not contain vertices from $W$ (otherwise $t$ would be reachable form $w$). Therefore augmenting on $P$ cannot change flow (and respectively, residual capacities) on edges $(V, W)$.
%\end{proof}

%
%\par
%We first convert the preflow $f$ on $E_R$ to an equivalent flow. First note, that increasing capacity of edges $(v,s)$ to the source or capacity of edges $(t,v)$to the sink leaves the value of all $s{-}t$ cuts unchanged. Indeed, \eg. an edge $(v,s)$ can never contribute to the cost of an $s{-}t$ cut, since $s$ is always in the source set.
%\par
%For each vertex $w$ in $R$ with excess $e(w)>0$ we increase capacity of the edge $(w,s)$ by $e(w)$ and increase the flow $f(w,s)$ by $e(w)$. For each vertex $w$ in $R$ with deficit $e(w)<0$ we increase capacity of the edge $(t,w)$ by $-e(w)=|e(w)|$ and increase the flow $f(t,w)$ by $-e(w)$.
%\par
%This way all the excess and deficit is returned to the source and sink and $f$ is a valid flow in $E_R$. For an edge $(s,w)$ there will appear a residual capacity $c_f(s,w) = \max(e(w),0)$ and for edge $(w,t)$ a residual capacity $c_f(w,t) = \max(-e(w),0)$.
%\par
%%
%
%\begin{myalgorithm}{Augmented Path Region Discharge}
%\label{alg1}
%\item {\bf Input:} Region $R$ with boundary $B$. Pseudoflow $f$ on $E_R$, distance $d$ on $B$.
%\item Convert preflow $f$ to an equivalent flow.
%\item\hspace{1cm} Augment on paths $s\rightarrow t$ until no exist
%\item{\bf for} $k$ =1\dots n-1
%\item\hspace{1cm} Augment on paths $s\rightarrow \{v\in B\mid d(v)=k\}$ until no exist
%%\item\hspace{1cm} {\bf for} $v\in B \mid\ d(v)=k$ 
%%\item\hspace{2cm} \add an edge $(v,t)$ with capacity $\infty$ and length $k$.
%%\item\hspace{1cm} Augment on paths $s\rightarrow v$ until no exist
%%\item\hspace{1cm} {\bf end}
%\item{\bf end}
%\item\label{A1 relable} Compute $d$ on $R$ by region-relabel
%\end{myalgorithm}
%
%
If the network has integer capacities, algorithm terminates in a finite number of iterations.
\begin{statement}[Correctness]
Alg.~\ref{alg1} outputs a stable preflow-labeling.
\end{statement}
\begin{proof}
Because the output labeling is the residual sink distance, it is stable. We need to show that preflow is stable. 
\par
Let us show that push is not applicable in $s$. Let $T_k = \{t\}\cup \{v\in B \mid d(v)\leq k\}$. On the step $l\geq k$ source is disconnected from $T_k$. Let $v\in T_k$, on the step $k = d(v)$, $s$ is disconnected from $v$. By Lemma 1 this property is persistent.
\par
After the region relabel (line~\ref{A1 relable}) all nodes from which $T_n$ is not reachable gain label $n$ and hence there is no $w$ such that $c_f(s,w)>0$ and $d(w)<n$.
\par
The algorithm creates flow excess on the boundary. It remains to show that boundary nodes are stable.
\par
Let $v\in B$, let $d(v)=k$. On the beginning of step $k$ there is no path $s\rightarrow T_{k-1}$, so either 1) there is no path $s\rightarrow v$ either 2) there is no path $v\rightarrow T_{k-1}$.
\begin{enumerate}
\item There is no path to $v$ on any further step of the algorithm (Lemma 1), therefore no augmentation to $v$ will take place and $e(v)=0$ on step $n$ so $v$ is stable.
\item $T_{k-1}$ will remain unreachable from $v$ and $s$ until the end of the algorithm and on step $n$ we have that for any $w$ such that $c_f(v,w)>0$ $d(w)>=k$.
\end{enumerate}
\end{proof}
\par
\begin{myalgorithm}{Region Distributed maxflow}
\label{fullalg}
\item Input: network $G$ %, region cover $R$: $\cup R_i = V$
\item {\bf while} network is not stable
\item\hspace{1cm} Take one or several disjoint regions of $V$ and perform RegionDischarge in parallel
\item\hspace{1cm} update flow on boundaries
\item\hspace{1cm} update labels
\item\hspace{1cm} update label histogram
\item {\bf end}
\end{myalgorithm}
\par
\begin{statement}Algorithm~\ref{fullalg} terminates in a finite number of steps. Give standard bound.
\end{statement}
\begin{proof}
The distributed algorithm terminates when all regions are stable. This will happen in a finite number of iterations as after each region discharge a node either becomes an excess node either its label is increased at least by 1.
\end{proof}
\begin{statement}Labeling $d$ is a lower bound on the distance to sink in $G$.
\end{statement}
\begin{proof}
By construction.
\end{proof}
From this statement we conclude an important property,
\begin{statement}\label{source set}
When a vertex $v$ reaches the label $n$ during RegionDischarge, then
\begin{itemize}
\item There exist a minimal cut $(\bar T,T)$ such that $v\in \bar T$.
\item If $v$ is reachable from any excess node, then for any minimal cut $(S,\bar S)$ it holds $v\in S$.
\end{itemize}
%it necessarily belongs to the source set $S$ of any minimal cut.
\end{statement}
\begin{proof}
A vertex $v$ may only reach label $n$ when it is disconnected from the sink and from all boundary vertices of $R$, therefore it is disconnected from the sink in $G$. It will stay disconnected from the sink upon termination of the algorithm. At this point sink cut $(\bar T, T)$, $T =\{w| \exists w\rightarrow t\}$ is optimal and we have $v \in \bar T$.
\par
{\bf todo: part 2}
\par
After flushing the excesses $e$ back to source there will appear a path $s\rightarrow v$. This path will never be augmented during the further execution of the algorithm, therefore any minimal cut cannot cross $s\rightarrow v$, that is $v$ must be in the source set.
\end{proof}
\par
\subsection{Augmenting Path Pseudoflow Discharge}
In the intermediate steps of the algorithm we identified some vertices which may be optimally assigned to the source set of the cut by Statement~\ref{source set}. Such vertices do not take part in the further computation and may be safely removed together with all their neighboring edges. This would free memory for other vertices and the region $R$ can be enlarged. However, we can do better and identify also vertices which necessarily belong to the sink set. Next we show a modified algorithm which allows to identify both while serving as a basic operation for a preflow-push.
\par
\begin{myalgorithm}{Augmented Path Pseudoflow Region Discharge}
\label{alg2}
%\item Construct network $G_R$ of vertices $R^+$, edges $(R,V)$, edges $(s,B^+)$ carrying the excess and edges $(B^-,t)$ carrying the deficit and converting the preflow $f$ to a flow on $G_R$. 
\item {\bf Input:} Region $R$, boundary $B$. Pseudoflow $f$ on $E_R$, distance $d$ on $B$.
\item Convert preflow $f$ to an equivalent flow.
\item\label{A2augment} augment on paths $s\rightarrow t$
\item\label{boundary split} source boundary $B^S = \{v| v\in B, \exists s\rightarrow v\}$
\item[] sink boundary $B^T = \{v| v\in B, \exists v\rightarrow t\}$
\item\label{A2 augment S} augment on paths $s\rightarrow v$, $v\in B^S$ in order of increasing labels of $v$.
\item\label{A2 augment T} augment on paths $B^T \rightarrow t$
\item Compute $d_{-}(R)$ and $d_{+}(R)$ by pseudoflow region-relabel
\item Perform pseudoflow gap heuristic
\item {\bf if} $d_{-}(v)=n$ and $d_{+}(v)<n$ assign $v$ to $S$ and remove from $G$
\item {\bf if} $d_{-}(v)<n$ and $d_{+}(v)=n$ assign $v$ to $T$ and remove from $G$
\item group vertices with $d_{+}(v)=d_{-}(v)=n$ into connected components, assign each component to either $S$ or $T$ and remove it from $G$.
\end{myalgorithm}
\par
\begin{statement}
Sets $B^S$ and $B^T$ constructed in step~\ref{boundary split} are disjoint.
\end{statement}
\begin{proof}
We have that $t$ is not reachable from $s$ after step~\ref{A2augment}. Assume $v$ in both $B^S$ and $B^T$, then there exist a path $s\rightarrow v \rightarrow t$, a contradiction.
\end{proof}
After step~\ref{A2augment} network $G_R$ is split into two disconnected network: with nodes reachable from $s$ and nodes from which $t$ is reachable. Therefore any augmentations occurring in steps \ref{A2 augment S} and \ref{A2 augment T} act on their respective subnetworks and can be carried independently of each other. As step~\ref{A2 augment S} doing the same work as Alg.~\ref{alg1}, all statemnt about alg~\ref{alg1} apply. The step~\ref{A2 augment T} implies also the following property. %, in particular Statement \ref{source set}.
\begin{statement}\label{sink set}
When a vertex $v$ get assigned sink label $d_{-}(v)=n$ during Pseudoflow region discharge, then
\begin{itemize}
\item There exist a minimal cut $(S,\bar S)$ such that $v\in \bar S$.
\item If any deficit node is reachable from $v$, then for any minimal cut $(S, \bar S)$ it holds $v\in \bar S$.
\end{itemize}
\end{statement}
\begin{proof}
\end{proof}
\par
\begin{myalgorithm}{Pseudoflow Region Distributed maxflow}
\label{fullalg}
\item Input: network $G$ %, region cover $R$: $\cup R_i = V$
\item {\bf while} network is not stable
\item\hspace{1cm} Take one or several disjoint regions of $V$ and perform Pseudoflow Region Discharge in parallel
%\item\hspace{1cm} Exclude 
\item\hspace{1cm} update flow on boundaries
\item\hspace{1cm} update labels
\item\hspace{1cm} update label histogram
\item {\bf end}
\end{myalgorithm}



\section{Complexity Analysis with Fixed Regions}

\begin{definition}[Region Discharge] An operation is called Region Discharge of $R$ if it satisfies the follwoing:\\
{Input}: Network $G$, labeling $d$ -- lower bound on distance in $G$\\
{Result}: flow $f$ in $G^R$ and labeling $d'$
\begin{compactenum}
\item\label{RD-flow} $f$ is maximum flow in $G^R$ %no path $s \rightarrow t$ in $G^R_f$
\item\label{RD-monotone} $d' \geq d$; $d' = d$ outside $R$
\item\label{RD-LB} $d'$ is lower bound on distance in $G_{f}$
\item\label{RD-out} $\forall (u,v)\in E^R,\, v\in B$ \  $\big(f(u,v)> 0 \Rightarrow d(u)>d(v)\big)$
%\item $d' \geq d$
\end{compactenum}
\end{definition}
Let us verify that Alg.\,\ref{RD-PR} is a Region Discharge operation according to this definition. Indeed, push operations applied to $v\in R$ modify only edges of the region network, so $f$ is a flow in $G^R$. There is no active vertices, so $f$ is maximal in $G^R$. Labels are never decreased and push operation preserves the lower bound property~\cite{GT88}. The property~\ref{RD-out} follows from the conditions of push operation -- the preflow is always pushed to a vertex with lower label.
\par
%While the algorithm of~\cite{Delong08} allows selecting regions dynamically during the run time, we will analyze the case when the regions are fixed. In this case it is possible to prove a tighter bound on number of region discharges, although in practice dynamic regions could be of advantage. 

%We will leave for later the discussion about how the sequential for loop in step 3 can run 
A straightforward bound on the number of sweeps can be obtained as follows. In each sweep every active node is touched at least once, therefore the proof in~\cite{Goldberg-PhD} for parallel push-relabel applies and gives a bound of $O(n^2)$ sweeps.
\par
We will prove a tighter bound.


==> tex/vision_results.tex <==
\begin{longtable}{|lcc|c|c|c|c|ccc|ccc|}
\caption[Problems from~\url{http://vision.csd.uwo.ca/maxflow-data/}]{Problems from~\url{http://vision.csd.uwo.ca/maxflow-data/}} \label{table1} \\
\hline
\multicolumn{3}{|c|}{problem} & BK & HIPR0 & HIPR0.5 & HPR & \multicolumn{3}{|c|}{S-ARD} & \multicolumn{3}{|c|}{S-PRD}\\* 
\hline
\rowcolor{blue!10}
 name & n($10^6)$ & m/n & CPU & CPU & CPU & CPU & CPU & \hskip-1mm sweeps\hskip-1mm &  $K$  & CPU & \hskip-1mm sweeps\hskip-1mm &   $K$ \\* 
\rowcolor{blue!10}
 size &         &     & RAM & RAM & RAM & RAM & RAM &    & I/O & RAM &    & I/O\\* 
\endfirsthead
\multicolumn{13}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\hline
\endhead
\hline \multicolumn{13}{|r|}{{Continued on next page}} \\ \hline
\endfoot
\hline \hline
\endlastfoot
\hline
\multicolumn{13}{|c|}{\bf stereo}\\* 
\hline 
\showrowcolors
\rowcolor{blue!10}
BVZ-sawtooth(20) & $0.2$ & $4.0$ & $0.68$s & $3.0$s & $7.7$s & $3.8$s & $0.62$s & $  6$ & $ 16$ & $2.7$s & $ 26$ & $ 16$ \\* 
\showrowcolors
\rowcolor{blue!10}
\multicolumn{3}{|>{\columncolor[rgb]{0.9,0.9,1}}l|}{434$\times$380, \ \ $ 14$MB} & $ 14$MB &  &  & $ 17$MB & $1.3{+}14.2$MB & &  & $0.7{+}1.1$MB & & $0.6$GB\\ 
\hiderowcolors
BVZ-tsukuba(16) & $0.1$ & $4.0$ & $0.36$s & $1.9$s & $4.9$s & $2.6$s & $0.34$s & $  5$ & $ 16$ & $1.7$s & $ 23$ & $ 16$ \\* 
\hiderowcolors
\multicolumn{3}{|l|}{384$\times$288, \ \ $8.6$MB} & $9.7$MB &  &  & $ 11$MB & $1.0{+}9.6$MB & &  & $0.5{+}0.7$MB & & $349$MB\\ 
\showrowcolors
\rowcolor{blue!10}
BVZ-venus(22) & $0.2$ & $4.0$ & $1.2$s & $5.7$s & $15$s & $6.2$s & $1.1$s & $  6$ & $ 16$ & $5.8$s & $ 29$ & $ 16$ \\* 
\showrowcolors
\rowcolor{blue!10}
\multicolumn{3}{|>{\columncolor[rgb]{0.9,0.9,1}}l|}{434$\times$383, \ \ $ 14$MB} & $ 15$MB &  &  & $ 17$MB & $1.5{+}14.3$MB & &  & $0.7{+}1.1$MB & & $0.8$GB\\ 
\hiderowcolors
KZ2-sawtooth(20) & $0.3$ & $5.8$ & $1.8$s & $7.1$s & $22$s & $6.1$s & $2.1$s & $  6$ & $ 16$ & $6.0$s & $ 21$ & $ 16$ \\* 
\hiderowcolors
\multicolumn{3}{|l|}{$ 38$MB} & $ 33$MB &  &  & $ 36$MB & $3.5{+}31.8$MB & &  & $1.5{+}2.3$MB & & $1.1$GB\\ 
\showrowcolors
\rowcolor{blue!10}
KZ2-tsukuba(16) & $0.2$ & $5.9$ & $1.1$s & $5.3$s & $20$s & $4.4$s & $1.4$s & $  6$ & $ 16$ & $5.4$s & $ 15$ & $ 16$ \\* 
\showrowcolors
\rowcolor{blue!10}
\multicolumn{3}{|>{\columncolor[rgb]{0.9,0.9,1}}l|}{$ 26$MB} & $ 23$MB &  &  & $ 25$MB & $2.6{+}22.1$MB & &  & $1.1{+}1.6$MB & & $0.5$GB\\ 
\hiderowcolors
KZ2-venus(22) & $0.3$ & $5.8$ & $2.8$s & $13$s & $39$s & $10$s & $3.4$s & $  8$ & $ 16$ & $12$s & $ 29$ & $ 16$ \\* 
\hiderowcolors
\multicolumn{3}{|l|}{$ 38$MB} & $ 34$MB &  &  & $ 37$MB & $3.5{+}32.9$MB & &  & $1.5{+}2.4$MB & & $1.5$GB\\ 
\hline
\multicolumn{13}{|c|}{\bf multiview}\\* 
\hline 
\showrowcolors
\rowcolor{blue!10}
BL06-camel-lrg & $18.9$ & $4.0$ & $81$s &  &  &  & $63$s & $ 11$ & $ 16$ & $308$s & $418$ & $ 16$ \\* 
\showrowcolors
\rowcolor{blue!10}
\multicolumn{3}{|>{\columncolor[rgb]{0.9,0.9,1}}l|}{100$\times$75$\times$105$\times$24, \ \ $2.0$GB} & $1.6$GB &  &  &  & $ 19{+}103$MB & & $ 28$GB & $ 86{+}122$MB & & $0.6$TB\\ 
\hiderowcolors
BL06-camel-med & $9.7$ & $4.0$ & $25$s & $29$s & $77$s & $59$s & $20$s & $ 12$ & $ 16$ & $118$s & $227$ & $ 16$ \\* 
\hiderowcolors
\multicolumn{3}{|l|}{80$\times$60$\times$84$\times$24, \ \ $1.0$GB} & $0.8$GB &  &  & $1.0$GB & $ 31{+} 53$MB & & $ 16$GB & $ 46{+} 63$MB & & $225$GB\\ 
\showrowcolors
\rowcolor{blue!10}
BL06-camel-sml & $1.2$ & $4.0$ & $0.98$s & $1.5$s & $6.3$s & $1.8$s & $0.96$s & $  9$ & $ 16$ & $4.2$s & $ 47$ & $ 16$ \\* 
\showrowcolors
\rowcolor{blue!10}
\multicolumn{3}{|>{\columncolor[rgb]{0.9,0.9,1}}l|}{40$\times$30$\times$42$\times$24, \ \ $115$MB} & $106$MB &  &  & $124$MB & $8.0{+}7.0$MB & & $1.4$GB & $6.9{+}8.2$MB & & $9.1$GB\\ 
\hiderowcolors
BL06-gargoyle-lrg & $17.2$ & $4.0$ & $245$s &  &  & $91$s & $154$s & $ 21$ & $ 16$ & $318$s & $354$ & $ 16$ \\* 
\hiderowcolors
\multicolumn{3}{|l|}{80$\times$112$\times$80$\times$24, \ \ $1.8$GB} & $1.5$GB &  &  & $1.7$GB & $ 23{+} 95$MB & & $ 35$GB & $ 82{+}112$MB & & $0.8$TB\\ 
\showrowcolors
\rowcolor{blue!10}
BL06-gargoyle-med & $8.8$ & $4.0$ & $115$s & $17$s & $58$s & $37$s & $73$s & $ 16$ & $ 16$ & $143$s & $340$ & $ 16$ \\* 
\showrowcolors
\rowcolor{blue!10}
\multicolumn{3}{|>{\columncolor[rgb]{0.9,0.9,1}}l|}{64$\times$90$\times$64$\times$24, \ \ $0.9$GB} & $0.8$GB &  &  & $0.9$GB & $ 37{+} 50$MB & & $ 14$GB & $ 44{+} 58$MB & & $235$GB\\ 
\hiderowcolors
BL06-gargoyle-sml & $1.1$ & $4.0$ & $6.1$s & $1.2$s & $3.0$s & $1.7$s & $4.1$s & $  9$ & $  9$ & $4.4$s & $ 55$ & $  9$ \\* 
\hiderowcolors
\multicolumn{3}{|l|}{32$\times$45$\times$32$\times$24, \ \ $106$MB} & $ 97$MB &  &  & $114$MB & $ 14{+} 99$MB & &  & $6.9{+}7.7$MB & & $9.4$GB\\ 
\hline
\multicolumn{13}{|c|}{\bf surface}\\* 
\hline 
\showrowcolors
\rowcolor{blue!10}
LB07-bunny-lrg & $49.5$ & $6.0$ &  &  &  &  & $15$s & $  6$ & $ 64$ & $416$s & $ 43$ & $ 64$ \\* 
\showrowcolors
\rowcolor{blue!10}
\multicolumn{3}{|>{\columncolor[rgb]{0.9,0.9,1}}l|}{401$\times$396$\times$312, \ \ $6.6$GB} & $5.7$GB &  &  &  & $130{+} 87$MB & & $ 49$GB & $226{+} 99$MB & & $276$GB\\ 
\hiderowcolors
LB07-bunny-med & $6.3$ & $6.0$ & $1.6$s & $20$s & $41$s & $26$s & $2.0$s & $  9$ & $ 64$ & $16$s & $ 27$ & $ 64$ \\* 
\hiderowcolors
\multicolumn{3}{|l|}{202$\times$199$\times$157, \ \ $0.8$GB} & $0.7$GB &  &  & $0.8$GB & $ 81{+}714$MB & &  & $ 43{+}863$MB & & $0.0$MB\\ 
\showrowcolors
\rowcolor{blue!10}
LB07-bunny-sml & $0.8$ & $5.9$ & $0.17$s & $0.80$s & $1.8$s & $1.1$s & $0.32$s & $  9$ & $ 64$ & $0.91$s & $ 19$ & $ 64$ \\* 
\showrowcolors
\rowcolor{blue!10}
\multicolumn{3}{|>{\columncolor[rgb]{0.9,0.9,1}}l|}{102$\times$100$\times$79, \ \ $ 94$MB} & $ 95$MB &  &  & $101$MB & $8.2{+}1.6$MB & & $0.8$GB & $7.9{+}115.9$MB & & $0.0$MB\\ 
\hline
\multicolumn{13}{|c|}{\bf segm}\\* 
\hline 
\hiderowcolors
liver.n26c10 & $4.2$ & $10.4$ & $6.4$s & $18$s & $18$s & $34$s & $14$s & $ 13$ & $ 64$ & $39$s & $157$ & $ 64$ \\* 
\hiderowcolors
\multicolumn{3}{|l|}{170$\times$170$\times$144, \ \ $2.1$GB} & $0.8$GB &  &  & $0.7$GB & $ 36{+} 12$MB & & $ 13$GB & $ 30{+} 13$MB & & $ 82$GB\\ 
\showrowcolors
\rowcolor{blue!10}
liver.n26c100 & $4.2$ & $11.1$ & $12$s & $26$s & $28$s & $39$s & $24$s & $ 15$ & $ 64$ & $35$s & $ 98$ & $ 64$ \\* 
\showrowcolors
\rowcolor{blue!10}
\multicolumn{3}{|>{\columncolor[rgb]{0.9,0.9,1}}l|}{170$\times$170$\times$144, \ \ $2.1$GB} & $0.8$GB &  &  & $0.7$GB & $ 38{+} 13$MB & & $ 16$GB & $ 30{+} 14$MB & & $ 66$GB\\ 
\hiderowcolors
liver.n6c10 & $4.2$ & $9.8$ & $7.2$s & $17$s & $25$s & $40$s & $14$s & $ 16$ & $ 64$ & $36$s & $151$ & $ 64$ \\* 
\hiderowcolors
\multicolumn{3}{|l|}{170$\times$170$\times$144, \ \ $498$MB} & $0.7$GB &  &  & $0.7$GB & $ 65{+}659$MB & &  & $ 28{+} 13$MB & & $ 79$GB\\ 
\showrowcolors
\rowcolor{blue!10}
liver.n6c100 & $4.2$ & $10.5$ & $15$s & $30$s & $34$s & $44$s & $19$s & $ 17$ & $ 64$ & $32$s & $ 94$ & $ 64$ \\* 
\showrowcolors
\rowcolor{blue!10}
\multicolumn{3}{|>{\columncolor[rgb]{0.9,0.9,1}}l|}{170$\times$170$\times$144, \ \ $512$MB} & $0.8$GB &  &  & $0.7$GB & $ 35{+} 12$MB & & $ 14$GB & $ 29{+} 13$MB & & $ 70$GB\\ 
\hiderowcolors
babyface.n26c10 & $5.1$ & $47.3$ &  &  &  &  & $179$s & $ 38$ & $ 64$ & $222$s & $169$ & $ 64$ \\* 
\hiderowcolors
\multicolumn{3}{|l|}{250$\times$250$\times$81, \ \ $2.5$GB} & $3.7$GB &  &  &  & $156{+} 56$MB & & $102$GB & $173{+} 58$MB & & $0.6$TB\\ 
\showrowcolors
\rowcolor{blue!10}
babyface.n26c100 & $5.1$ & $49.0$ &  &  &  &  & $231$s & $ 44$ & $ 64$ & $262$s & $116$ & $ 64$ \\* 
\showrowcolors
\rowcolor{blue!10}
\multicolumn{3}{|>{\columncolor[rgb]{0.9,0.9,1}}l|}{250$\times$250$\times$81, \ \ $2.7$GB} & $3.8$GB &  &  &  & $156{+} 56$MB & & $115$GB & $180{+} 57$MB & & $0.6$TB\\ 
\hiderowcolors
babyface.n6c10 & $5.1$ & $11.1$ & $6.8$s & $38$s & $51$s & $68$s & $20$s & $ 17$ & $ 64$ & $100$s & $275$ & $ 64$ \\* 
\hiderowcolors
\multicolumn{3}{|l|}{250$\times$250$\times$81, \ \ $0.6$GB} & $1.0$GB &  &  & $0.9$GB & $ 22{+} 16$MB & & $ 19$GB & $ 37{+} 17$MB & & $261$GB\\ 
\showrowcolors
\rowcolor{blue!10}
babyface.n6c100 & $5.1$ & $11.5$ & $13$s & $71$s & $65$s & $87$s & $24$s & $ 19$ & $ 64$ & $74$s & $191$ & $ 64$ \\* 
\showrowcolors
\rowcolor{blue!10}
\multicolumn{3}{|>{\columncolor[rgb]{0.9,0.9,1}}l|}{250$\times$250$\times$81, \ \ $0.6$GB} & $1.0$GB &  &  & $0.9$GB & $ 22{+} 16$MB & & $ 18$GB & $ 37{+} 17$MB & & $189$GB\\ 
\hiderowcolors
adhead.n26c10 & $12.6$ & $31.5$ &  &  &  &  & $128$s & $ 17$ & $ 64$ & $224$s & $109$ & $ 64$ \\* 
\hiderowcolors
\multicolumn{3}{|l|}{256$\times$256$\times$192, \ \ $6.5$GB} & $6.2$GB &  &  &  & $153{+} 83$MB & & $ 84$GB & $195{+} 86$MB & & $0.8$TB\\ 
\showrowcolors
\rowcolor{blue!10}
adhead.n26c100 & $12.6$ & $31.6$ &  &  &  &  & $174$s & $ 21$ & $ 64$ & $269$s & $129$ & $ 64$ \\* 
\showrowcolors
\rowcolor{blue!10}
\multicolumn{3}{|>{\columncolor[rgb]{0.9,0.9,1}}l|}{256$\times$256$\times$192, \ \ $6.7$GB} & $6.3$GB &  &  &  & $153{+} 83$MB & & $ 90$GB & $196{+} 86$MB & & $0.8$TB\\ 
\hiderowcolors
adhead.n6c10 & $12.6$ & $11.6$ &  &  &  &  & $36$s & $ 13$ & $ 64$ & $119$s & $161$ & $ 64$ \\* 
\hiderowcolors
\multicolumn{3}{|l|}{256$\times$256$\times$192, \ \ $1.6$GB} & $2.5$GB &  &  &  & $ 34{+} 36$MB & & $ 31$GB & $ 77{+} 39$MB & & $372$GB\\ 
\showrowcolors
\rowcolor{blue!10}
adhead.n6c100 & $12.6$ & $11.7$ &  &  &  &  & $49$s & $ 20$ & $ 64$ & $121$s & $165$ & $ 64$ \\* 
\showrowcolors
\rowcolor{blue!10}
\multicolumn{3}{|>{\columncolor[rgb]{0.9,0.9,1}}l|}{256$\times$256$\times$192, \ \ $1.6$GB} & $2.5$GB &  &  &  & $ 34{+} 36$MB & & $ 36$GB & $ 77{+} 39$MB & & $354$GB\\ 
\hiderowcolors
bone.n26c10 & $7.8$ & $32.3$ &  &  &  &  & $25$s & $ 12$ & $ 64$ & $96$s & $148$ & $ 64$ \\* 
\hiderowcolors
\multicolumn{3}{|l|}{256$\times$256$\times$119, \ \ $3.9$GB} & $4.0$GB &  &  &  & $122{+} 61$MB & & $ 35$GB & $147{+} 63$MB & & $470$GB\\ 
\showrowcolors
\rowcolor{blue!10}
bone.n26c100 & $7.8$ & $32.4$ &  &  &  &  & $29$s & $ 14$ & $ 64$ & $68$s & $124$ & $ 64$ \\* 
\showrowcolors
\rowcolor{blue!10}
\multicolumn{3}{|>{\columncolor[rgb]{0.9,0.9,1}}l|}{256$\times$256$\times$119, \ \ $4.1$GB} & $4.0$GB &  &  &  & $122{+} 61$MB & & $ 39$GB & $147{+} 63$MB & & $321$GB\\ 
\hiderowcolors
bone.n6c10 & $7.8$ & $11.5$ & $7.7$s & $5.7$s & $17$s & $12$s & $7.2$s & $  9$ & $ 64$ & $37$s & $195$ & $ 64$ \\* 
\hiderowcolors
\multicolumn{3}{|l|}{256$\times$256$\times$119, \ \ $0.9$GB} & $1.5$GB &  &  & $1.4$GB & $ 62{+} 23$MB & & $ 13$GB & $ 52{+} 25$MB & & $188$GB\\ 
\showrowcolors
\rowcolor{blue!10}
bone.n6c100 & $7.8$ & $11.6$ & $9.1$s & $9.1$s & $22$s & $14$s & $8.7$s & $ 10$ & $ 64$ & $23$s & $ 65$ & $ 64$ \\* 
\showrowcolors
\rowcolor{blue!10}
\multicolumn{3}{|>{\columncolor[rgb]{0.9,0.9,1}}l|}{256$\times$256$\times$119, \ \ $1.0$GB} & $1.6$GB &  &  & $1.5$GB & $ 62{+} 23$MB & & $ 13$GB & $ 52{+} 25$MB & & $104$GB\\ 
\hiderowcolors
bone\_subx.n6c100 & $3.9$ & $11.8$ & $7.1$s & $6.3$s & $12$s & $6.4$s & $5.5$s & $ 12$ & $ 64$ & $9.4$s & $ 42$ & $ 64$ \\* 
\hiderowcolors
\multicolumn{3}{|l|}{128$\times$256$\times$119, \ \ $495$MB} & $0.8$GB &  &  & $0.7$GB & $ 39{+} 12$MB & & $7.1$GB & $ 29{+} 13$MB & & $ 42$GB\\ 
\showrowcolors
\rowcolor{blue!10}
bone\_subxy.n26c100 & $1.9$ & $32.2$ & $5.9$s & $3.9$s & $6.1$s & $4.6$s & $7.3$s & $ 13$ & $ 64$ & $8.7$s & $ 33$ & $ 64$ \\* 
\showrowcolors
\rowcolor{blue!10}
\multicolumn{3}{|>{\columncolor[rgb]{0.9,0.9,1}}l|}{128$\times$128$\times$119, \ \ $1.0$GB} & $1.0$GB &  &  & $0.8$GB & $ 92{+}851$MB & &  & $ 50{+} 16$MB & & $ 39$GB\\ 
\hiderowcolors
abdomen\_long.n6c10 & $144.4$ & $11.8$ &  &  &  &  & $179$s & $ 11$ &  &  & $>35$ &  \\* 
\hiderowcolors
\multicolumn{3}{|l|}{512$\times$512$\times$551, \ \ $ 19$GB} & $ 29$GB &  &  &  & $410{+}403$MB & & $196$GB &  & & ${>}1$TB\\ 
\showrowcolors
\rowcolor{blue!10}
abdomen\_short.n6c10 & $144.4$ & $11.8$ &  &  &  &  & $82$s & $ 11$ &  &  &  &  \\* 
\showrowcolors
\rowcolor{blue!10}
\multicolumn{3}{|>{\columncolor[rgb]{0.9,0.9,1}}l|}{512$\times$512$\times$551, \ \ $ 19$GB} & $ 29$GB &  &  &  & $410{+}403$MB & & $138$GB &  & & \\ 
\hline 
\end{longtable} 

